2D Points Curve Reconstruction Survey and Benchmark

Curve reconstruction from unstructured points in a plane is a fundamental problem with many applications that has generated research interest for decades. Involved aspects like handling open, sharp, multiple and non-manifold outlines, run-time and provability as well as potential extension to 3D for surface reconstruction have led to many different algorithms. We survey the literature on 2D curve reconstruction and then present an open-sourced benchmark for the experimental study. Our unprecedented evaluation on a selected set of planar curve reconstruction algorithms aims to give an overview of both quantitative analysis and qualitative aspects for helping users to select the right algorithm for specific problems in the field. Our benchmark framework is available online to permit reproducing the results, and easy integration of new algorithms.

==> sec/4_shape.tex <==

\subsection{Boundaries of Dot Patterns}


\JP{Overview}
~\cite{Funke:2006:HDM:1137856.1137911}

\todo{TODOs: An image showing the results of alpha shape, chi shape, ~\cite{PEETHAMBARAN2015164}, ~\cite{METHIRUMANGALATH201590}, other algos}.

%\subsection{Delaunay Filtering}\label{subsec:shape_del}
In a survey on shape reconstruction, Edelsbrunner elaborates on how different shape reconstruction methods restrict the Delaunay complex to arrive at their respective shapes \cite{10.1007/BFb0054315}. In $\mathbb{R}^{2}$, $\alpha$-shapes of a point set $S$ is generated by connecting the points $p$,$q$ $\in$ $S$, which are touched by an empty disk of radius $\alpha$ \cite{edelsbrunner83alpha}. However, $\alpha$-shape construction is parameterized in terms of $\alpha$ and there exists some point sets for which the $\alpha$-shape family does not contain elements representing appropriate shapes \cite{Melkemi20001423}. To overcome the limitations of $\alpha$-shape, Melkemi has introduced $\mathbf{\emph{A}}$-shapes \cite{Melkemi20001423} which contains $\alpha$-shape and crust \cite{amenta98curve} as special cases. Given a finite set of points $P$, and an arbitrarily chosen set $A$, $\mathbf{\emph{A}}$-shape of $P$ is generated by first constructing the Voronoi diagram for $A\cup P$ and then joining together any pair of points $p$,$q$ $\in P$ whose Voronoi cells border each other and border some common Voronoi cell containing a point of $A$. However, determination of a proper $A$ in $\mathbf{\emph{A}}$-shape computation is controlled by two parameters, $\alpha$ and $t$.

A related notion for characterizing a point set distribution is characteristic shape (or $\chi$-shape) \cite{DUCKHAM20083224}. $\chi$-shape algorithm removes external edges of Delaunay triangulation until the largest edge on the boundary is less than a threshold value. Termination and efficiency of the algorithm and the boundary of $\chi$-shape are dependent on the threshold value. Further, it generates only simply connected shapes (holes cannot be detected). Recently, variants of $\alpha$-shapes such as k-order $\alpha$-hulls \cite{KRASNOSHCHEKOV201476} and LDA-$\alpha$-complex \cite{Chevallier:2011:BNP:1998196.1998278} have been proposed for shape reconstruction. LDA-$\alpha$-complex effectively uses the local density variation found in the point sets for detecting the hollow regions.

~\cite{PEETHAMBARAN2015164}, ~\cite{METHIRUMANGALATH201590}, ~\cite{METHIRUMANGALATH2017124}

%\subsection{Border Extraction}\label{subsec:shape_other}
A related line of work is polygonal border extraction of dot patterns which are mainly used in pattern recognition and digital image processing \cite{Chaudhuri1997257}. Chaudhuri et al. \cite{Chaudhuri1997257} introduced two new constructs called as $s$-shape and $r$-shape for border extraction. In 1999, Gautam et al. \cite{Garai199975} proposed a split and merge procedure for computing the polygonal border of a dot pattern. Their final polygonal border depends on the choice of the number of sides of final polygon(\emph{m}) or the area of the polygonal border. Recently, a polygonal border reconstruction algorithm (simple shape) has been proposed by A.Gheibi et al., which works for both dot patterns and boundary samples \cite{simpleshape}. However, simple shape depends on a thresh hold parameter and lacks the ability to detect holes in the shapes.

%\subsection{Region Boundaries}\label{subsec:shape_region} 
Many GIS applications require the boundary approximation of certain points of interests or region. Researchers have utilized the counter part of convex hull to capture region boundaries.  In this direction, Junyi Xu et al. \cite{5648277} propose $\omega$-hull algorithm to compute concave hull for scattered data based on Graham scan convex hull algorithm. As the name suggests, the concave hull generated depends on the value of two externally supplied parameters, $\omega$ and $\rho$. A $\emph{k}$-nearest neighbor algorithm for computing concave hull of point sets can be found in \cite{DBLP:conf/grapp/MoreiraS07}. This is essentially a modified Gift wrapping algorithm which produces an envelope for a set of points where the shape of the envelope depends on the value of $\emph{k}$. Galton et al. \cite{10.1007/11863939_6} presented a swinging arm algorithm for the computation of region occupied by set of points in plane. The footprint obtained by Swinging Arm algorithm depends on the value of swinging arm, which is a line anchored to the last point added to the footprint. However, unlike convex hull, concave hull lacks a concrete mathematical definition and thus result in non-unique representations for boundaries of planar point sets.


~\cite{song2010boundary},  , ~\cite{ZHU2017178}, ~\cite{Chevallier:2011:BNP:1998196.1998278}, ~\cite{nguyen08vicur}


%------------------------------------------------------------------------- 

==> sec/item.tex <==
\begin{figure*}
\centering
\begin{overpic} 
[width=\linewidth]
% [width=\linewidth,grid,tics=10]
{\currfiledir/figure.png}
\put(0,-1){\todo{\currfiledir}}
\end{overpic}
\caption{
% 
% 
Algorithm outline:
(a) the contact-behavior of two implicit surfaces is annotated by the user;
(b) annotations probe the implicit functions generating a set of samples;
(c) an operator template $\bar{g}$ is deformed onto these samples, generating an optimized surface-operator $\tilde{g}$;
(d) the deformed template generates the blending function $g$ through smooth optimization;
(e) the operator can be used to re-produce the desired contact behavior. 
% 
% 
}
% \todo{start from some example meshes (a), sample the scalar fields on the surface of the examples (b), fit the optimal curve (c) to produce the corresponding composition operator (d).}}
\label{fig:pipeline}
\end{figure*}

